Fibrations of algebras

We study fibrations arising from indexed categories of the following form: fix two categories $\mathcal{A},\mathcal{X}$ and a functor $F : \mathcal{A} \times \mathcal{X} \longrightarrow\mathcal{X} $, so that to each $F_A=F(A,-)$ one can associate a category of algebras $\mathbf{Alg}_\mathcal{X}(F_A)$ (or an Eilenberg-Moore, or a Kleisli category if each $F_A$ is a monad). We call the functor $\int^{\mathcal{A}}\mathbf{Alg} \to \mathcal{A}$, whose typical fibre over $A$ is the category $\mathbf{Alg}_\mathcal{X}(F_A)$, the "fibration of algebras" obtained from $F$. Examples of such constructions arise in disparate areas of mathematics, and are unified by the intuition that $\int^\mathcal{A}\mathbf{Alg} $ is a form of semidirect product of the category $\mathcal{A}$, acting on $\mathcal{X}$, via the `representation' given by the functor $F : \mathcal{A} \times \mathcal{X} \longrightarrow\mathcal{X}$. After presenting a range of examples and motivating said intuition, the present work focuses on comparing a generic fibration with a fibration of algebras: we prove that if $\mathcal{A}$ has an initial object, under very mild assumptions on a fibration $p : \mathcal{E}\longrightarrow \mathcal{A}$, we can define a canonical action of $\mathcal{A}$ letting it act on the fibre $\mathcal{E}_\varnothing$ over the initial object. This result bears some resemblance to the well-known fact that the fundamental group $\pi_1(B)$ of a base space acts naturally on the fibers $F_b = p^{-1}b$ of a fibration $p : E \to B$.

==> fouche/alphabets.tex <==
\ExplSyntaxOn

\clist_new:N \g_fouche_upper_clist
\clist_gset:Nn \g_fouche_upper_clist { A,B,C,D,E,F,G,H,I,J,K,L,M,N,O,P,Q,R,S,T,U,V,W,X,Y,Z }

\clist_new:N \g_fouche_lower_clist
\clist_gset:Nn \g_fouche_lower_clist { a,b,c,d,e,f,g,h,i,j,k,l,m,n,o,p,q,r,s,t,u,v,w,y,z }

\clist_new:N \g_fouche_both_clist
\clist_concat:NNN \g_fouche_both_clist \g_fouche_upper_clist \g_fouche_lower_clist

\clist_new:N \g_fouche_categories_clist
\clist_gset:Nn \g_fouche_categories_clist { Ab, Adj, LAdj, RAdj, Fib, Tw, coAlg, Opt, Lens, Seq, Alg, Ban, BSD, Card, cat, Cat, CAT, cgHaus, Ch, CMnd, CMon, CW, Der, EM, End, Ext, fHilb, Fld, Foo, Fuk, fVect, coEM, Fzy, Gal, Grp, gVec, Haus, Het, Ho, Kl, Lat, Mag, Met, Mfd, Mod, Mly, Mre, Mon, Ord, Par, PInj, Lie, CCHopf, POrd, Pre, Pro, Prof, Psd, opFib, Quot, Quux, coKl, Rel, Ring, Rot, Set, Sgp, Sp, Spec, sSet, Sub, SW, Top, Tor, Unif, Vect, ArithCat, AbCat, SAbCat, PNat, CWd, Wd, DiNat }

\clist_new:N \g_fouche_operators_clist
\clist_gset:Nn \g_fouche_operators_clist { lan, Lan, LAN, lft, Lft, LFT, Nat, ran, Hom, Ran, RAN, Rft, Yan, RFT, rft, op, co, coop, colim, coker, }

\cs_new_protected:Npn \fouche_makeabbrev:nnN #1 #2 #3
{
	\clist_map_inline:Nn { #3 }
	{
		\cs_new_protected:cpn { #2 } { #1 { ##1 } }
	}
}
\fouche_makeabbrev:nnN { \mathbf } { bf#1 } \g_fouche_both_clist
\fouche_makeabbrev:nnN { \boldsymbol } { bs#1 } \g_fouche_both_clist
\fouche_makeabbrev:nnN { \mathsf } { sf#1 } \g_fouche_both_clist
\fouche_makeabbrev:nnN { \mathfrak } { fk#1 } \g_fouche_both_clist
\fouche_makeabbrev:nnN { \underline } { un#1 } \g_fouche_both_clist

\fouche_makeabbrev:nnN { \mathcal } { cl#1 } \g_fouche_upper_clist
\fouche_makeabbrev:nnN { \mathbb } { bb#1 } \g_fouche_upper_clist

\fouche_makeabbrev:nnN { \mathsf } { #1 } \g_fouche_categories_clist
\fouche_makeabbrev:nnN { \mathrm } { #1 } \g_fouche_operators_clist

\DeclareMathAlphabet{\mybb}{U}{BOONDOX-ds}{m}{n}
\fouche_makeabbrev:nnN { \mybb } { mb#1 } \g_fouche_lower_clist
\ExplSyntaxOff


==> fouche/envs.tex <==
\DeclareOption{english}{
	\theoremstyle{definition}
	\numberwithin{equation}{section}
	\newtheorem{theorem}{Theorem}[section]
	\defthm{corollary}{Corollary}
	\defthm{proposition}{Proposition}
	\defthm{lemma}{Lemma}
	\defthm{claim}{Claim}
	\defthm{question}{Question}
	\defthm{definition}{Definition}
	\defthm{notation}{Notation}
	\defthm{result}{Result}
	\defthm{remark}{Remark}
	\defthm{conjecture}{Conjecture}
	\defthm{axiom}{Axiom}
	\defthm{example}{Example}
	\defthm{examples}{Examples}
	\defthm{exercise}{Exercise}
	\defthm{counterexample}{Counterexample}
	\defthm{construction}{Construction}
	\defthm{warning}{Warning}
	\defthm{digression}{Digression}
	\defthm{perspective}{Perspective}
	\defthm{discussion}{Discussion}
	\defthm{terminology}{Terminology}
	\defthm{heuristics}{Heuristics}
	\defthm{conclusion}{Conclusion}
	\defthm{assumption}{Assumption}
}

\makeatletter
\def\renewtheorem#1{%
	\expandafter\let\csname#1\endcsname\relax
	\expandafter\let\csname c@#1\endcsname\relax
	\gdef\renewtheorem@envname{#1}
	\renewtheorem@secpar
}
\def\renewtheorem@secpar{\@ifnextchar[{\renewtheorem@numberedlike}{\renewtheorem@nonumberedlike}}
\def\renewtheorem@numberedlike[#1]#2{\newtheorem{\renewtheorem@envname}[#1]{#2}}
\def\renewtheorem@nonumberedlike#1{
	\def\renewtheorem@caption{#1}
	\edef\renewtheorem@nowithin{\noexpand\newtheorem{\renewtheorem@envname}{\renewtheorem@caption}}
	\renewtheorem@thirdpar
}
\def\renewtheorem@thirdpar{\@ifnextchar[{\renewtheorem@within}{\renewtheorem@nowithin}}
\def\renewtheorem@within[#1]{\renewtheorem@nowithin[#1]}
\makeatother

\makeatletter
\def\redefthm#1#2{%
	\renewtheorem{#1}{#2}[section]%
	\expandafter\def\csname #1autorefname\endcsname{#2}%
	\expandafter\let\csname c@#1\endcsname\c@theorem}
\makeatother

\DeclareOption{italian}{
	\theoremstyle{definition}
	\numberwithin{equation}{section}
	\renewtheorem{theorem}{Teorema}[section]
	\redefthm{corollary}{Corollario}
	\redefthm{proposition}{Proposizione}
	\redefthm{lemma}{Lemma}
	\redefthm{definition}{Definizione}
	\redefthm{notation}{Notazione}
	\redefthm{remark}{Osservazione}
	\redefthm{conjecture}{Congettura}
	\redefthm{axiom}{Assioma}
	\redefthm{example}{Esempio}
	\redefthm{examples}{Esempi}
	\redefthm{exercise}{Esercizio}
	\redefthm{exercises}{Esercizi}
	\redefthm{counterexample}{Controesempio}
	\redefthm{construction}{Costruzione}
	\redefthm{warning}{Caveat}
	\redefthm{digression}{Digressione}
	\redefthm{perspective}{Prospettiva}
	\redefthm{discussion}{Discussione}
	\redefthm{terminology}{Terminologia}
	\redefthm{heuristics}{Euristica}
}

\DeclareDocumentEnvironment{enumtag}{m O{}}{%
	\begin{enumerate}[ label = \textsc{#1}\oldstylenums{\arabic*}), ref   = \textsc{#1}\oldstylenums{\arabic*}, #2] }{ \end{enumerate} }


==> fouche/macros.tex <==
\def\To{\Rightarrow}
\usepackage{svg}
\newcommand{\arXivlogo}{%
	\includesvg[scale=0.12]{arxiv-logo}%
}
\newcommand{\arXivPreprint}[1]{
	\href{http://arxiv.org/abs/#1}{arXiv:#1}%{\raisebox{-3pt}{\arXivlogo}}%
}


\newlength{\seplen}
\setlength{\seplen}{5pt}
\newlength{\sepwid}
\setlength{\sepwid}{.4pt}
\def\firstblank{\,\rule{\seplen}{\sepwid}\,}
\def\sndblank{\firstblank\llap{\raisebox{2pt}{\firstblank}}}

\newcommand{\celtag}[2][dr]{\ar[#1,white, "#2"{black,description}]}


\let\xto\xrightarrow
\let\xot\xleftarrow

\newcommand{\rot}[3][c]{\rotatebox[origin=#1]{#2}{$#3$}}
\newcommand{\rotarrow}[2][c]{\rot{#1}{#2}{\Rightarrow}}

\providecommand{\Nearrow}{\rotarrow{45}}
\providecommand{\Nwarrow}{\rotarrow{135}}
\providecommand{\Searrow}{\rotarrow{-45}}
\providecommand{\Swarrow}{\rotarrow{225}}
\providecommand{\Sarrow}{\rotarrow{-90}}
\providecommand{\Narrow}{\rotarrow{90}}

\newcommand{\bsmat}{\begin{smallmatrix}}
		\newcommand{\esmat}{\end{smallmatrix}}

\makeatletter
\def\@cite#1#2{[\textsf{#1}\if@tempswa , #2\fi]}
\def\@biblabel#1{[\textsf{#1}]}
\makeatother


\newcommand{\falgFun}{\rtimes}

% Objects of a category
\newcommand{\Ob}[1]{\mathsf{Ob}(#1)}

% Pairing of objects (using the univ. prop. of products)
\newcommand{\pairing}[2]{\langle {#1}, {#2} \rangle}
% CoPairing of objects (using the univ. prop. of coproducts)
\newcommand{\coPair}[2]{[ {#1}, {#2} ]}
% CoPairing of objects (as a left adjoint to pairing)
\newcommand{\coPairSum}[2]{[ {#1}, {#2} ]}
% CoPairing of objects (as a right adjoint to pairing)
\newcommand{\coPairTimes}[2]{[ {#1}, {#2} ]}

\newcommand{\pto}{\mathop{\ooalign{\hfil\kern-2pt$\mapstochar$\hfil\cr\hfil$\to$\hfil}}}

\usepackage{turnstile}
\newcommand{\adjunct}[2]{\nsststile{#2}{#1}}

\newcommand{\putbib}[2]{
	\bibliography{#1}{}
	\bibliographystyle{#2}
}

\usetikzlibrary{decorations.markings}
\tikzstyle{pro} =
[ decoration={ markings
		, mark = at position 0.5 with
			{\draw[-] (0,-1.25pt) -- (0,1.25pt);}
	}
, postaction ={decorate}
]

\newcommand*{\Scale}[2][4]{\scalebox{#1}{\ensuremath{#2}}}%
\def\lrc{
	\begin{tikzpicture}[scale=.33]
		\draw[-] (0,0) -| (1,1);
	\end{tikzpicture}
}

\def\dopb{\begin{tikzpicture}[scale=.375,-] \draw (0,0) -| (1,1);\end{tikzpicture}}
\newcommand{\xpb}[1][dr]{\ar@{}[#1]|(.375){\dopb}}
\def\dopo{\begin{tikzpicture}[scale=.375] \draw (0,0) |- (1,1);\end{tikzpicture}}
\newcommand{\xpo}[1][dr]{\ar@{}[#1]|(.675){\dopo}}

\newcommand{\pb}{\arrow[dr, phantom, "\dopb", very near start]}
\newcommand{\po}{\arrow[dr, phantom, "\dopo", very near end]}

\def\[{\begin{equation}}
			\def\]{\end{equation}}
% ^ this is BAD, but can't do without at this point...

\newenvironment{xsmallmatrix}[1]
{\renewcommand\thickspace{\kern#1}\smallmatrix}
{\endsmallmatrix}

\NewDocumentCommand{\prevar}{o m m}{
	\IfNoValueTF{#1}{
		\begin{smallmatrix}
			#2 \\
			\downarrow \\
			#3
		\end{smallmatrix}}
	{
		\begin{xsmallmatrix}{0em}
			& #2 \\
			#1 & \downarrow \\
			& #3
		\end{xsmallmatrix}}}

\ExplSyntaxOn
\NewDocumentCommand{\var}{ o m m }{
	\IfNoValueTF{#1}
	{#2 \fib #3}
	{#1 : #2 \fib #3}
	}
\newcommand{\precop}[2]{
	\begin{smallmatrix}
		#1 \\ #2
	\end{smallmatrix}
}
\NewDocumentCommand{\cop}{O{r} m m}{
	\str_case:nn { #1 } {
		{r}{\left( \precop{#2}{#3}\right)}
		{s}{\left[ \precop{#2}{#3}\right]}
		{c}{\left\{ \precop{#2}{#3}\right\}}
		{a}{\left\langle \precop{#2}{#3}\right\rangle}
	}}

\ExplSyntaxOff

\usepackage{adjustbox}
\newenvironment{adju}[1][0.925]{%
	\begin{center}\begin{adjustbox}{max height=0.5\textheight, max width=#1\textwidth}}{\end{adjustbox}\end{center}}

% Formatting for category names like /Set, /Cat and so on.
\newcommand{\catFont}[1]{\mathsf{#1}}

\def\emdash{\text{-}}
\NewDocumentCommand{\VCat}{ O{\clV} }{#1\emdash\Cat}
\def\twoCat{\VCat[2]}

\newcommand{\adja}[4]{
	#1 : \xymatrix{#2 \ar@<.5em>[r] \ar@{}[r]|\perp & \ar@<.5em>[l] #3 } : #4
}


\NewDocumentCommand{\vxy}{o m}{
	\IfNoValueTF{#1}
	{\vcenter{\xymatrix{#2}}} % do if \vxy{bla}
	{\vcenter{\xymatrix#1{#2}}} % do if \vxy[foo]{bla}
}

\newcommand\mapsfrom{\mathrel{\raisebox{.1em}{\rotatebox[origin=c]{180}{$\mapsto$}}}}
%{\mathrel{\reflectbox{\ensuremath{\mapsto}}}}

% \newcommand{\de}{\partial}
% \NewDocumentCommand{\FMly}{ O{} }{\IfNoValueTF{#1}{F\emdash\Mly}{F^{#1}\emdash\Mly}}
% \NewDocumentCommand{\FMre}{ O{} }{\IfNoValueTF{#1}{F\emdash\Mre}{F^{#1}\emdash\Mre}}
% \newcommand{\dMly}{\de\emdash\Mly}
% \newcommand{\dMre}{\de\emdash\Mre}

\newcommand{\params}{\clA} % The category of parameters
\newcommand{\carriers}{\clX} % The category of carriers
\newcommand{\fibTotal}{\clE} % The total category of a fibration
\newcommand{\fib}{\twoheadrightarrow}
\newcommand{\param}{A}
\newcommand{\carrier}{X}

% Notation for an algebra of a parameterized monad
% \alg{param}{carrier}{structure}
\newcommand{\alg}[3]{(#2,#3)^{#1}}
\newcommand{\coalg}[3]{(#2,#3)_{#1}}



%\newcommand{\monad}[1]{\mathbf{#1}}

\newcommand{\Mnd}[1]{\catFont{Mnd}(#1)} % The category of monads on #1
\newcommand{\coMnd}[1]{\catFont{coMnd}(#1)} % The category of comonads on #1

% Action of A on X
\newcommand{\act}[2]{#1 \cdot #2}

% The 2-category of parametric monads with category of parameters #1
\newcommand{\ParMnd}[1]{\catFont{ParMnd}(#1)}
\newcommand{\ParMndInit}[1]{\catFont{ParMnd}_\initial(#1)}
\newcommand{\ParCoMndInit}[1]{\catFont{ParCoMnd}_\initial(#1)}

% The 2-category of nice fibrations.
\newcommand{\niceFib}[1]{\catFont{pFib}(#1)}
\newcommand{\niceOpFib}[1]{\catFont{pOpFib}(#1)}
% \newcommand{\niceFib}[1]{\catFont{Fib}_{\initial,\terminal}(#1)}
% \newcommand{\niceOpFib}[1]{\catFont{opFib}_{\terminal,\terminal}(#1)}

% Some sort of a slice 2-category. (pseduo?)
\newcommand{\niceSlice}[2]{#1/#2}

% 
\newcommand{\niceMnd}[1]{\Mnd{#1}_{\initial,\params}}
\newcommand{\niceCMnd}[1]{\CoMnd{#1}_{\terminal,\params}}
%\newcommand{\FibLR}[1]{\catFont{Fib}\ladj{}\radj{}(#1)}

\newcommand{\AlgOrCoAlg}{\catFont{(co)Alg}}

% The Grothendieck construction of contravariant pseudofunctors
\newcommand{\grothCont}[2][]{\int^{#1}#2}
% The Grothendieck construction of covariant pseudofunctors
\newcommand{\grothCov}[2][]{\int_{#1}#2}

% The total category of a fibration of algebras
% \algTotal[\monad]{\params}{\carriers}
\newcommand{\algTotal}[3][]{#2 \ltimes^{#1} #3}
% The total category of an opfibration of coalgebras
% \coalgTotal[\comonad]{\params}{\carriers}
\newcommand{\coalgTotal}[3][]{#2 \ltimes_{#1} #3}

\newcommand{\coCartCat}{\cate{coCartCat}}

\def\toprove{\fosco{This$\uparrow$ will require a proof}}
\NewDocumentCommand{\TP}{ O{A} m }{
i_R(p_L #1 + i#2)
}

% The fibre over #2 of a fibration #1
\newcommand{\fibre}[2]{#1_{#2}}

% The initialFibre of a fibration
\newcommand{\initialFibre}[1]{\fibre{#1}{\initial}}

% A morphism of fibrations
\newcommand{\fibMor}{h}
% A morphism of fibrations, restricted to a morphism between the initial fibres
\newcommand{\fibMorInit}{\fibmor_\initial}
\newcommand{\fibMorTwo}{\chi}

% A fibration morphism consisting of a 1-cell #1 and a 2-cell #2
\newcommand{\fibrationMorphism}[2]{(#1,#2)}

% A morphism of parametrized monads consists of
% a functor between the carrier categories
\newcommand{\mndMorCar}{u}
% a functor between the parameter categories
\newcommand{\mndMorPar}{v}
% and a mediator 2-cell
\newcommand{\mndMorTwo}{\delta}

% A monad morphism consisting of a 1-cell #1 and a 2-cell #2
\newcommand{\monadMorphism}[2]{(#1,#2)}

% The main adjunction
\newcommand{\mainAdj}{\Phi}

% The mate of a 2-cell
\newcommand{\mate}[1]{#1^+}

% Adjunctions over #1, meaning adjunctions whose induced moand lies on #1.
%\newcommand{\Adj}[1]{\cate{Adj}(#1)}

% For an opfibration, the reindexing functor along #1
%\newcommand{\opFibReindex}[1]{#1_{!}}
\newcommand{\opFibReindex}[1]{\Sigma_{#1}}

% For a fibration, the reindexing functor along #1
\newcommand{\fibReindex}[1]{#1^{\ast}}

% The unique morphism from the initial object
\newcommand{\fromInitial}{!}

\newcommand{\EMpseudofun}{\EM}

% A generic pseudofunctor B^op -> Cat
\newcommand{\pseudofunGeneric}{\clE_{(\firstblank)}}

% A generic pseudofunctor B^op -> Cat applied to an argument.
\newcommand{\pseodofunGenericAp}[1]{\clE_{#1}}

% The compositor of a pseudofunctor or an (op)lax functor
\newcommand{\compositor}{\kappa}



==> fouche/packages.tex <==

\RequirePackage{amsthm}
\RequirePackage[svgnames]{xcolor}
\RequirePackage{ amsfonts
	, amsmath
	, amssymb
	% , caption
	, epigraph
	, enumitem
	, lipsum
	, mathtools
	, hyphenat
	, tensor
	, todonotes
	, stackrel
	, tikz
	, hyperref
	, savesym
	, setspace
	, tikz-cd
	, tcolorbox
	, booktabs
	, multirow
	, verbatim
	% , calligra
	, url
}
\RequirePackage[all,2cell]{xy}\UseAllTwocells

% setup of specific packages

\usetikzlibrary{calc}
\usetikzlibrary{matrix,arrows}

\hypersetup{ %hyperfootnotes=true%
	, bookmarksnumbered=true%
	, bookmarksopen=true%
	, breaklinks=true%
	, urlcolor=black%
	, colorlinks%
	, citecolor=black%
	, linkcolor=black%
	, urlcolor=black%
}

\tikzset{commutative diagrams/.cd,arrow style=tikz,diagrams={>=Straight Barb}}


==> fouche/page-layout.tex <==
%per le formule nei titoli
%-------------------------------------------------------------------------
% \makeatletter
% \g@addto@macro\bfseries{\boldmath}
% \makeatother
%-------------------------------------------------------------------------

\makeatletter
\def\defthm#1#2{%
	\newtheorem{#1}{#2}[section]%
	\expandafter\def\csname #1autorefname\endcsname{#2}%
	\expandafter\let\csname c@#1\endcsname\c@theorem}
\makeatother

\tcbuselibrary{most}
\tcolorboxenvironment%
{quote}{ blanker
	, before skip=10pt
	, after skip=10pt
	, borderline west={6mm}{5pt}{gray!15}
	, breakable
}

\setcounter{tocdepth}{1}


==> sections/app-dump.tex <==

\section{A characterization, and on semidirect products}
\greta{Add new intro here}

\subsection{Parametricity via the product, and limits}\label{subsec:parametricity}
While it is natural to define fibrations of algebras through the application of the Grothendieck construction to a pseudofunctor, at times one might need alternative approaches; some are quite more elegant and allow for equivalent characterizations of fibrations of algebras.

Every parametrized functor ${F  : \params \too \en{\carriers}}$ induces an endofunctor
\[
	\hat{F}  \coloneqq (\pi_\params,F)  : \params \times \carriers \too \params \times \carriers \,, \quad (\param,\carrier) \mapsto (\param,F_\param\carrier)
\]
and the endofunctors $\hat{F}$ that are of this form are precisely the ones fibered over the projection in the sense of making the triangle
\[\vxy{
	\params \times \carriers
	\ar[rr]^{\hat{F}}
	\ar[dr]_{\pi_\params}
	& & \params \times \carriers
	\ar[dl]^{\pi_\params} \\
	& \params &
	}\]
commute.\footnote{A technical point: for practical reasons, we only ask the triangles in the slice-2-category to commute up to isomorphism.} As trivial as this observation might seem, it hides an elegant characterization: $\pi_\params$ is the trivial bundle over $\params$, \ie a specifically simple object
of the slice $2$-category $\Cat/\params$.

From this point of view, parametrized monads $T  : \params \too \Mnd{\carriers}$ correspond to monads
in the slice-2-category $\Cat/\params$, on the projection functor $\pi_\params  : \params \times \carriers \to \params$ (an \emph{object} of $\Cat/\params$). Thus, fibrations of algebras
form but a subclass of the formal theory of monads in the sense of \cite{Street1972}. This enables us to make immediate use of the theory and results that come for free when one studies 2-categories of monads, and their algebras.
\begin{theorem} \label{theorem:_product_presentation}
	The \textEM fibration $p^T  : \algTotal{\params}{\carriers} \fib \params$ of a parametrized monad $T  : \params \too \Mnd{\carriers}$ is equivalent, in the slice-2-category $\Cat/\params$, to
	\[
		\EM(\hat{T}) \xrightarrow{U^{\hat{T}}}\params \times \carriers \xrightarrow{\pi_\params} \params \,,
	\]
	where $U^{\hat{T}}$ is the forgetful functor from the category of  \textEM algebras of the monad
	\[
		\hat{T}  : \params \times \carriers  \too \params \times \carriers \,, \quad (\param,\carrier) \mapsto (\param, T_\param\carrier) .
	\]
	The functor $\var[p^T]{\algTotal{\params}{\carriers}}{\params}$ is also the (internal) \textEM object of the monad $\hat{T}$ in the slice-2-category $\Cat/\params$, on the projection $\var[\pi_\params]{{\params \times \carriers}}{\params}$.
\end{theorem}
\begin{proof}
	Clearly algebras for $\EM(\hat{T})$ are of the kind $(\id[\param],\xi) : (\param,T_\param \carrier)\to(\param,\carrier)$ with $\xi$ a $T_\param$ algebra, and similarly for their morphisms. The obvious correspondence
	\[
		(\param,\carrier,\xi : T_\param \carrier\to\carrier)\leftrightarrows(\id[\param],\xi : T_\param \carrier\to\carrier)
	\]
	makes an equivalence in $\Cat/\params$.
	As for the second part, we show its universal property. First of all consider  in $\Cat/\params$ the following 2-cell $\beta : \hat{T} U^{\hat{T}} \Rightarrow U^{\hat{T}}$,
	\[\vxy{
		\algTotal{\params}{\carriers}
		\ar[dr]_{{p^T}}
		\ar[r]^{U^{\hat{T}}}
		\ar@/^2pc/[rr]^{U^{\hat{T}}}
		&
		\params \times \carriers
		\ar[r]^{\hat{T}}
		\ar[d]_{\pi_\params}
		&
		\params \times \carriers\lltwocell<\omit>{<3>\beta}
		\ar[dl]^{\pi_\params} \\
		& \params
		}\]
	then we only need to show that it, together with $U^{\hat{T}}$, for any given $g : \clG\to\params$ induces a natural isomorphism between 1-cells in $H : g \to p ^T$ and $\hat{T}$-modules $(M : g\to\pi_\params,\lambda : \hat{T}\circ M\Rightarrow M)$. On one hand, each $H$ induces the module $(U^{\hat{T}}H, H\ast\beta)$ by composition and whiskering. On the other, a given module $(M,\lambda)$ for each $G$ and $MG=(\param_{G},\carrier_{G})$ defines a morphism $\lambda_G=(\id,\lambda_G^\carriers) : (\param_{G},T_{\param_{G}}\carrier_{G})\mapsto(\param_{G},\carrier_{G})$; then we can define a functor $H : G\mapsto (\param_{G},\carrier_{G},\lambda_G^\carriers)$. One can check that each of the two constructions provides a 1-cell in $\Cat/\params$, and they are one inverse to the other by definition of $\beta$. Everything is natural in $g$.
\end{proof}
From this characterization, it immediately follows that,
\begin{proposition} \label{proposition:_limits}
  Let $T : \params\too \Mnd{\carriers}$ be a parametric monad. Then, the forgetful functor
	\[
    \algTotal[T]{\params}{\carriers} \to \params \times \carriers , \quad (\carrier,\xi)^A \mapsto (\param,\carrier)
	\]
	is monadic, and therefore it creates limits.
\end{proposition}
As a corollary, we get an explicit way to compute limits in $\algTotal[T]\params\carriers$.
%\ulo{TODO: merge the two remarks}
%
%\begin{remark}\label{explicit_way_limits}
  %\color{red}
	%Using standard results about \textEM algebras, we now know how to calculate limits in $\algTotal{\params}{\carriers}$ using limits in $\carriers$ and in $\params$, since the forgetful functor $\algTotal{\params}{\carriers} \to \params \times \carriers$ creates limits. 
	
	%There is also a different way of calculating limits in $\algTotal{\params}{\carriers}$ that involves the fibration structure on $p^T$.
	%Let $D : \clJ \to \algTotal{\params}{\carriers}$ be a functor; its components given by $\alg{\param_j}{\carrier_j}{\xi_j}$.

	%If the morphisms $\alpha_J \colon A \to A_j$ form a limiting cone on $p^T \circ D \colon \clJ \to \params$, we can use the functors $\alpha^*_j \colon \EM(T_{\param_j}) \to \EM(T_\param)$ to transport all the algebras $\algTotal{\params}{\carriers}$ into the fibre $\EM(T_\param)$.

	%One chan check that ... form a limiting cone in $\EM(T_A)$.

	%does however provide a different way of calculating limits in 
	%which is not immediate from the approach that uses the Grothendieck construction.  and we can consider the limits $F = \lim_J F_J$ of all parameters, as well as the algebras $\alpha_J^*(X_J,x_J)$, each of which is an $F$-algebra by change of base; it is a routine exercise to check that the limit $(X,x)$ of these objects in $\Alg_\clX(F)$ yields the limit of $D$. Considering how $\algTotal[F]\params\carriers$ and $\EltsAlg\carriers$, $\EltsEM\carriers$ relate via \eqref{pb_endo}, \eqref{pb_em}, a similar argument shows also how to compute limits in a fibration of algebras modelled on $F : \clA \too \en\clX$: given a diagram $\barealg\clA\clX$ with components $(A_J; X_J, x_J)$, compute the limit $A = \lim_J A_J$ of the parameters; reindex all $F_{A_J}$-algebras to make them $F_A$-algebras and compute the limit in that fibre.
%\end{remark}

\begin{remark}%\label{explicit_way_limits}
  %\color{blue}
	%Recalling how limits in \textEM categories of algebras are created, we now know how to calculate limits in $\algTotal{\params}{\carriers}$ using limits in $\carriers$ and in $\params$, something which is not immediate from the approach that uses the Grothendieck construction. 

  %The recipe to build limits goes as follows. 
  Let $D : \clJ\too \algTotal\params\carriers$ be a functor; its components are given by  $DJ= \alg{\param_J}{\carrier_J}{\xi_J}$. From this we can consider the limit $\param = \lim_J \param_J$ of all parameters, and from the terminal cone maps $\alpha_J : \param \too \param_J$ we obtain the algebras $\alpha_J^*(\alg{\param_J}{\carrier_J}{\xi_J})$, each of which is a $T_\param$-algebra. 
   Examining what we get, we find that the limit $\alg{\param}{\carrier}{\xi}$ of these objects \emph{computed in $\EM(T_\param)$} yields the limit of $D$.
   % (this can be verified by comparing to the limit we get from \autoref{proposition:_limits}). The same argument works for endofunctor algebras.% as well.
   %Considering how $\algTotal[F]\params\carriers$ and $\EltsAlg\carriers$, 
%    $\EltsEM\carriers$ relate via \eqref{pb_endo}, \eqref{pb_em}, a similar argument shows also how to compute limits in a fibration of algebras modelled on $F : \clA \too \en\clX$: given a diagram $\barealg\clA\clX$ with components $(A_J; X_J, x_J)$, compute the limit $A = \lim_J A_J$ of the parameters; reindex all $F_{A_J}$-algebras to make them $F_A$-algebras and compute the limit in that fibre.
\end{remark}

\begin{remark}\label{remark_on_endofu}
	Analogously to \autoref{theorem:_product_presentation}, parametrized endofunctors and parametrized pointed endofunctors can be characterized internally in $\Cat/\params$. For  parametrized endofunctors $F  : \params \too \en\carriers$ with no extra structure, there is an evident way of constructing the total category of the fibration of endofunctor algebras as the category of endofunctor algebras of the endofunctor
	\[\vxy[@R=0cm]{\hat F :\clA\times\clX \ar[r]& \clA\times\clX\\
			(A,X) \ar@{|->}[r] & (A,F_AX)}\]
	as an endo-1-cell of $(\params\times\carriers,\pi_\params)$ in the $2$-category $\Cat/\params$, and the $2$-categorical characterisation of $\algTotal[F]{\params}{\carriers}$ is that of an \emph{inserter} \cite[(4.1)]{kelly_1989} of the identity and $\hat{F}$ in $\Cat/\params$.
\end{remark}
\autoref{theorem:_product_presentation} paves the way to an additional characterisation theorem for parametrized monads (that easily dualizes to comonads and adapts to more general parametrized endofunctors):
\begin{theorem}\label{as_monads_in_cokl}
The following pieces of data are equivalent:
\begin{enumtag}{pm}
\item \label{pm_1} a parametrized monad $T : \clA\times\clX \too \clX$, \ie (upon currying) a functor $\clA\too\Mnd{\clX}$;
\item \label{pm_2} a monad $T : (\clA\times\clX, \pi_\clA) \too (\clA\times\clX, \pi_\clA)$ in the 2-category $\Cat/\clA$, over the object $(\clA\times\clX,\pi_\clA)$;
\item \label{pm_3} a monad $T : \clA\times\clX \ptoo \clX$ in the 2-coKleisli category of strict 2-algebras, for the 2-comonad $\clA\times\firstblank$, over the object $\clX$.
% \item \label{pm_4} a monad in the (domain of the) 2-fibration $\Cat \ltimes^\ell \Cat$ obtained in \autoref{yoink_a_2_fibration}.
\end{enumtag}
\end{theorem}
\begin{proof}
Clearly, a monad like in \ref{pm_1} is an endo-1-cell of $\clX$ in the 2-category of \ref{pm_3}. Now it is enough to observe that the unit and multiplication of a parametric monad $T : \clA\too\Mnd{\clX}$ can be seen as 2-cells $\eta : \pi_\clX\To T$ and $\mu : T\bullet T \To T$ where $\pi_\clX : \clA\times\clX \too\clX$ is the projection functor and
	\[\label{nobody_expects_cokl_0} T\bullet T :
\clA\times\clX \xto{\Delta\times\clX}
\clA\times\clA\times\clX \xto{\clA\times T}
\clA\times\clX \xto{T} \clX\]
is a coKleisli composition.

As for \ref{pm_2}, note that we have to require $T$ to be a monad in $\Cat/\params$ and not in \emph{fibrations} over $\params$, because the adjunction $\params\times\carriers \leftrightarrows \algTotal[T]\params\carriers$ splitting the monad in \ref{pm_2} isn't always internal to fibrations (not all Cartesian arrows are preserved). 
\end{proof}
An immediate corollary of \autoref{as_monads_in_cokl} is the following.
\begin{remark}[Distributive laws between parametric functors]
	\autoref{proposition:_limits}, and \ref{as_monads_in_cokl} even more, are quite useful in pinpointing the correct notion of \emph{distributive law} between parametric endofunctors $S,T$%:\clX\too \clX$
    . 
    Recall that the classical notion of distributive law consists of a `lax intertwiner' $\lambda : ST\To TS$ between functors $S$ and $T$, so that it is compatible with the respective structure of $S$ and $T$ (them being monad and monad; comonad and monad; monad and comonad, etc.; cf.\, \cite[Appendix C.1]{Aguiar2020} for a thorough discussion on the matter of intertwining $p$ monads and $q$ comonads).

	Now \autoref{as_monads_in_cokl} allows describing distributive laws between parametric moands as distributive laws between a monad $T : \clA\times\clX \too\clA\times\clX$ on $\pi_\clA$, and a monad $S : \clB\times\clY\too \clB\times\clY$ on $\pi_\clB$. Though perhaps unpleasant, unwinding what this latter characterisation boils down to is just a matter of bookkeeping the notation.
\end{remark}
\autoref{as_monads_in_cokl} yields a concise characterisation of the simple fibration as a coKleisli object: a fibration $\var[p]\clE\clA$ is equivalent to $\klalg\clA\clX$ (resp., $\coklalg\clA\clX$) if and only if it is the (co)Kleisli object of a monad fibred over the projection.

An immediate consequence of such a characterisation is that 
\begin{remark}[The universal property of the simple fibration]
The simple fibration of \autoref{fib_reg_rep} and \autoref{fib_reg_rep} of a Cartesian category has a universal property in the 2-category $\Cat/\clA$; it is the coKleisli object of the comonad
	\[\vxy[@R=0cm]{
(A,X)\ar@{|->}[rr] && (A,A\times X) \\
\clA\times\clA\ar[rr]\ar[dddddr]_{\pi_\clA} && \clA\times\clA \ar[dddddl]^{\pi_\clA}\\
&&\\&&\\&&\\&&\\
&\clA &
}\]
\end{remark}
\begin{remark}
We have a complementary intuition on this construction: mimicking what happens when a monoid $M$ acts on itself on the left under the map $m\mapsto \lambda x.\,mx$, we call $P$ of Example~\ref{fib_reg_rep} the \emph{regular representation} of the cartesian monoidal category $(\clX,\times)$ on itself. In fact, one can easily generalize the example with this latter, more algebraic, intuition in mind.
\end{remark}
\begin{remark}
Monadicity and \autoref{remark_on_endofu} allow for swift characterizations of op/fibrations of co/algebras as universal objects; for example, the total Mealy opfibration of \autoref{example_mealy} comes up as the object of $R$-coalgebras in $\Cat/(\clK^\op\times\clK)$ for the aforementioned endofunctor $R$, and thus as the inserter
\[\vxy{
		\Mly \drtwocell<\omit>{} \ar[r]^-V\ar[d]_V& (\clK^\op\times\clK)\times\clK \ar@{=}[d]\\
		(\clK^\op\times\clK)\times\clK \ar[r]_-R & (\clK^\op\times\clK)\times\clK.
	}\]
The discussion in this section and \autoref{theorem:_product_presentation} also form the basis of comparing arbitrary fibrations against fibrations of algebras. A fibration $(\fibTotal,p)$ is an \textEM fibration if and only if there exists a morphism $(\fibTotal,p) \too (\params \times \carriers, \pi_\params)$ in $\Cat/\params$ which is \emph{monadic}. In \autoref{theorem:_the_fibration-monad_adjunction}, we shall see how, given a suitably nice fibration $p$, one can construct the appropriate fibration of algebras to compare it against.
\end{remark}
\section{Completeness and cocompleteness results}
While our definitions comprise many examples, the reader may not yet be convinced of the fruitfulness of approaching algebras using tools from the theory of fibrations. In this section we heavily use it in order to prove results about adjoints to reindexing (cf. \autoref{subsec:adj_to_reidx}), about the existence of certain colimits and accessibility issues (cf. \autoref{subsec:colims}), and to finally argue in favour of our semidirect product notation (cf. \autoref{subsec:act}).

\todo[inline]{Fouche: metto una sezione nuova come separatore; da un punto di vista filosofico l'esistenza di aggiunti ai reindexing è un teorema di co/completezza, perché l'unico modo in cui lo dimostriamo è appellarci a un aft. Per il resto: invece l'intuizione come prodotto semidiretto è ottima ma non c'entra con i colimiti}
\subsection{Adjoints to reindexing, bifibrations and colimits}\label{subsec:adj_to_reidx}
Recall that a fibration is a bifibration if all the reindexing functors have left adjoints \cite[9.1.2]{CLTT}. While the reindexings of a fibration of algebras need not in general have left adjoints, they preserve all types of limits that exist in $\carriers$. To see that this is the case, simply observe that the reindexing functors make the triangles
\[\vxy{
	\Alg(G)
	\ar[rr]% ^{\hat{F}}
	\ar[dr] %_{\pi_\params}
	& & \Alg(F)
	\ar[dl] %^{\pi_\params}
   \\
	& \carriers &
	}\]
involving the (limit creating) forgetful functors commute. With the adjoint functor theorem in mind, therefore, a fibration of algebras is intuitively never very far from being a bifibration, the main obstruction being the lack of colimits in the fibres.

If we are dealing with \textEM algebras, we can make use of the standard fact that any comparison functor $\EM(T) \too \EM(S)$, induced by a monad morphism $S \To T$, has a left adjoint as soon as $\EM(T)$ has reflexive coequalizers.  

\begin{proposition} \label{prop:monad_algebra_bifibration}
Given a parametrized monad $\params \too \Mnd{\carriers}$, if all the fibres of the fibration $p^T \colon \algTotal{\params}{\carriers} \fib \params$ have reflexive coequalizers, then $p^T$ is a bifibration. 
\end{proposition}

In particular, if $\carriers = \Set$, the fibration of \textEM algebras is a bifibration.
Note that under the assumptions of \autoref{prop:monad_algebra_bifibration}, if the category $\carriers$ is additionally cocomplete, then Linton's construction of colimits of algebras \cite{Linton_coeqs} implies that the fibres of the fibration of Eilenberg-Moora algebras are all cocomplete as well.


% \begin{proposition}
% 	\label{prop:pres}Let $\clJ$ be a small category, and assume $\carriers$ admits $\clJ$-shaped limits; then the reindexing functor $\alpha^* : \Alg(G)\too \Alg(F)$ preserves limits of shape $\clJ$ for every $\alpha:F\To G$ in $\en\clX$.
% \end{proposition}

% \[\vxy{
% 	\Alg(G)
% 	\ar[rr]^{\hat{F}}
% 	\ar[dr]_{\pi_\params}
% 	& & \Alg(F)
% 	\ar[dl]^{\pi_\params} \\
% 	& \carriers &
% 	}\]
% While 


% \begin{corollary}
% 	If $\clX$ is complete then $\EltsAlg{\clX}$ is complete too and $\var[U]{\EltsAlg{\clX}}{\en\clX}$ preserves all limits.
% \end{corollary}

When dealing with endofunctor algebras, in order to make the situation more tractable, we start with the classifying case, namely with fibrations as in Example~\ref{subexam_algebras}, with some additional properties on the category $\clX$ (=that it is $\kappa$-accessible) and restricting to the functors $F\in\en\clX[<\kappa]$ (=the subcategory of $\kappa$-accessible functors), it is possible to employ a specific form of the adjoint functor theorem to prove the existence of left adjoints for each reindexing.
\begin{theorem}\label{swindle_theorem}
	Let $\clX$ be $\kappa$-presentable and assume that the fibration of algebras is restricted to just the $\kappa$-accessible functors $\clX\too \clX$, then each reindexing $\alpha^*$ has a left adjoint $\opFibReindex{\alpha}$.
\end{theorem}
\begin{proof}
	The proof follows an argument that we would like to call `Freyd swindle';%
	\footnote{The term `swindle' entered some parts of mathematical practice as a non-derogatory way to refer to `clever tricks, akin to sleights of hand, providing proofs of true statements based on illegal but evocative manipulations'. Example of this might be the offhanded re-bracketing of an infinite sum of real numbers (as in Euler's proofs of some analytic identities), or an infinite direct sums of $R$-modules, as in \cite[Corollary 2.7]{lamlam} where the term `Eilenberg swindle' was apparently coined, or of connected sums of compact manifolds, \cite{Tao_2009}.

		From our category-theoretic standpoint, the sleight of hand is instead a demonstration of stubbornness: to build a certain universal object, you apply a certain universal construction, for example a pushout. The pushout will hardly compute the desired left adjoint $\sum_\alpha(A,a)$. But one insists, and applies the same construction again, to the new piece of data; the pushout at this second stage will hardly be the desired $\sum_\alpha(A,a)$. But you insist, \dots{} and after a certain number of steps you get an answer in the form of a fix-point: in our case, $SP_\infty=S\left(\colim \dots\right)\cong\colim\, S\dots$ is the clever re-bracketing (but apart from a few little sins of omissions in what exactly the isomorphism means, the argument is totally rigorous).

		As for attributing the swindle to P.J. Freyd, more than one bright argument in his mathematical work is based on a similar technique of `doing one thing for a transfinite number of steps'.%
	} we sketch the idea in the case $\kappa=\omega$, for bigger ordinals one argues similarly.

	Let $\alpha^* : \Alg(G) \too \Alg(F) : \alg{G}{Y}{\zeta} \mapsto \alg{F}{X}{\alpha_X \circ \zeta}$ be the functor between algebras induced by a natural transformation $\alpha : F \To G$, and consider an $F$-algebra $\xi : FX\to X$; consider the pushout
	\[\vcenter{\xymatrix{
				FX \xpo \ar[r]^\alpha \ar[d]_{\xi} & GX \ar[d]\\
				X \ar[r]_{t_0}& P_0
			}}\]
	and define inductively the chain at the lower horizontal side of the diagram
	\[\vcenter{\xymatrix{
				FX \xpo \ar[r]^\alpha \ar[d]_{\xi} & GX \ar[r]^{Gt_0}\ar[d]\xpo & GP_0 \ar[r]^{Gt_1}\ar[d]\xpo& GP_1 \ar[d]\ar[r]&\dots \ar[r]\xpo & \boxed{?}\ar[d]\\
				X \ar[r]_{t_0}& P_0 \ar[r]_{t_1} & P_1 \ar[r]_{t_2} & P_2 \ar[r]_{t_3}&\dots\ar[r] & P_\infty
			}}\]
	The accessibility assumption on $G$ now implies that $GP_\infty$ is the colimit of the upper horizontal chain, so $\boxed{?}=GP_\infty$. The pushout cocone then yields a canonical choice of a map $\zeta_\infty : GP_\infty\to P_\infty$.
\end{proof}
% \begin{remark}
% 	Note that each reindexing having a left adjoint is equivalent to $U$ being a bifibration.
% \end{remark}


\subsection{Colimits in fibrations of algebras}\label{subsec:colims}

%\ulo{I separated the adjoints to reindexing stuff from colimit stuff into separate subsections. TODO: haven't adjusted the following section yet to account for this change.}

%\ulo{Really, the adjoints to reindexing and the colimit stuff should probably be in its own section not in the \textit{Alternative approaches to fibrations of algebras} section.}

\greta{Should really merge this subsection and the one before this -- faccio domani.

Meglio, va riarrangiata tutta la sezione.}

In Proposition~\ref{proposition:_limits} we obtained that limits in $\algTotal{\params}{\carriers}$ are created by a monadic functor $\algTotal{\params}{\carriers} \too \params \times\carriers$. Colimits in categories of algebras, on the other hand, are usually way more difficult to compute as, even when they exist, they tend to be complicated objects -- this is the case, for example, for initial endofunctor algebras.

The present subsection investigates two connected problems:
\begin{itemize}
	\item
	      how to induce/compute colimits in the total categories of the \textEM or endofunctor algebra fibrations?
	\item
	      how to ensure that reindexings (which preserve all limits, given the fact that these are created in the base) have left adjoints?
\end{itemize}

The second problem can be addressed looking at the `classifying' fibration of algebras
and then argue that some relevant property is preserved under pullback.

Let us start with the case of monads.
Leveraging on \cite[4.3.6]{Bor2} and on the fact that  $\algTotal\clA\clX$ is monadic over $\clA \times \clX$, one can prove very swiftly the following.
\begin{theorem}
	Let $T : \clA\too\Mnd{\clX}$ be a parametrized monad such that $T$ preserves filtered colimits in each variable separately; if $\clX$ is cocomplete, then so is $\algTotal\clA\clX$.
\end{theorem}

\begin{remark}
	In order to proceed with the discussion, let's make blanket assumptions the ones in \autoref{swindle_theorem}, \ie let's restrict the action of the pseudofunctor $F\mapsto \Alg(F)$ to accessible functors (and monads) defined on an accessible base category $\carriers$. More formally, we consider the accessible analogue of \eqref{pb_endo} and \eqref{pb_em}, \ie the pullbacks
	\[\vxy{
		(\algTotal{\en\carriers}{\carriers})_{<\kappa}\ar[r]\ar[d]_{U_{<\kappa}}\xpb & \algTotal{\en\carriers}{\carriers}\ar[d]^U &
		(\algTotal{\Mnd\carriers}{\carriers})_{<\kappa}\ar[r]\ar[d]_{U_{<\kappa}}\xpb & \algTotal{\Mnd\carriers}{\carriers}\ar[d]^U\\
		\en\carriers[<\kappa] \ar@{^{(}->}[r]& \en\carriers &
		\Mnd\carriers_{<\kappa} \ar@{^{(}->}[r]& \Mnd\carriers \\
		}\]
\end{remark}
Leveraging on the following result, we can prove that all fibrations obtained by pulling back the classifying fibration of algebras share its properties in terms of limit-preserving reindexings:
\begin{lemma}
	Let $\var[p]{\fibTotal}{\params}$ be a fibration such that each reindexing $\fibReindex{u} : \fibTotal_{\param'} \too \fibTotal_\param$ preserves (co)limits; let $F : \params' \too \params$ be a functor and $q$ the fibration obtained pulling back $p$ along $F$. Then, each reindexing of $q$ also preserves (co)limits.
\end{lemma}

\ulo{Move the lemma to the reindexing section.}

We are then left with the problem of establishing how colimits in each fibre $\falgFibre \param \carriers$ of a fibration of \textEM algebras for $T$ induce, if anything, \emph{global} colimits in the whole $\barealg\params\carriers$, provided some additional assumptions on $T$ are made. The issue is somewhat subtle, as it is well-known that being `internally' cocomplete as an object in $\Fib$ is a weaker property than having a cocomplete total category, \cite[p. 87]{streicher2023fibred}. Are total categories of fibrations of algebras cocomplete in the weak sense, or in the strong sense? And how does this relate to assumptions made on $\params,\carriers$ or $T : \params\times\carriers \too \carriers$?


One preliminary remark is the following well-known observation by Linton \cite{Linton_coeqs}: an \textEM category over a cocomplete base has coproducts as long as it has certain specific reflexive coequalisers, and it is cocomplete if it has all reflexive coequalisers.

\ulo{Join the previous and the following section.}

Computing such coequalisers is a difficult task in general, although a general recipe has been given by Linton \cite{Linton_coeqs}.
Calculations applying this general result provide us with the following.
\begin{proposition}\label{prop:fib_for_colim}
	In the specific case of $\algTotal\params\carriers$ regarded as an \textEM category (cf. \autoref{theorem:_product_presentation}), in the computation of binary coproducts, the coequaliser in question happens in a single fibre -- the one over  $A+B$, the coproduct in $\params$.
\end{proposition}
\begin{proof}
	Letting $*$ denote the coproduct of algebras, computing coequalisers in the specific case of $\algTotal\params\carriers$ regarded as an \textEM category goes as follows: given algebras $(X,\xi)$ and $(Y,\theta)$, their coproduct is the coequaliser of the reflexive pair
	\[\vxy[@C=1.4cm]{
		FUFU(X,\xi) * FUFU(Y,\theta) \ar@<.4em>[r]^-{\epsilon FU(X,\xi) * \epsilon FU(Y,\theta)} \ar@<-.4em>[r]_-{FU\epsilon_X * FU\epsilon_Y} & FU(X,\xi) * FU(Y,\theta)
		}\]
	where the coproduct of free algebras is simplified by the observation that $FUX*FUY\cong F(UX+UY)$ since $F$ is a left adjoint.

	In the specific case of $\emalg\clA\clX$ the coequaliser that defines the coproduct $(X,\xi)^A*(Y,\theta)^B$ is then
	\[\vxy[@C=1.4cm]{
			\big(T_{A+B}(T_AX+T_BY),\mu^{A+B}\big)^{A+B} \ar@<.4em>[r] \ar@<-.4em>[r]& \big(T_{A+B}(X+Y), \mu^{A+B} \big)^{A+B}
		}\]
	where it is not fundamental to make explicit what objects are involved, but rather that the coequaliser in question happens in a single fibre, the one over $A+B$ (coproduct in $\clA$). This colimit can't in general be reduced further (although there are cases where it acquires a more explicit form, for example when $A$ is the initial object of $\clA$).
\end{proof}
In light of this, our fibre-wise approach seems well justified. As in the case of \autoref{swindle_theorem}, additional properties on the categories involved make the problem more tractable, so much so that we can prove the following.

\begin{theorem}\label{thm:accessible}
	Let $\clA,\clX$ be both $\kappa$-accessible categories for some regular cardinal $\kappa$; furthermore, let all the parametrized functors $T_A$ that we consider be $\kappa$-accessible.
	Then the pseudofunctor $\Alg_\clX : \en\clX[<\kappa]^\op \too \Cat$ is accessible in the sense of \cite[5.3.1]{MP89}, which means that
	\begin{itemize}
		\item the base category and each fiber are accessible,
		\item each reindexing is an accessible functor,
    \item $\Alg_\clX(\colim\, T_i)\cong \lim_i \Alg_\clX(T_i)$ for every $\kappa$-filtered diagram $\clJ \too \en\carriers[<\kappa]$.%. : i\mapsto T_i$.
	\end{itemize}
\end{theorem}
\begin{proof}
	% \fosco{Expand on this}
	The category of $\kappa$-accessible functors $\en\clX[<\kappa]$ is itself accessible (although for a bigger cardinal $\lambda\gg\kappa$; if $\clX$ is $\kappa$-\emph{presentable} instead, the category $\en\clX[<\kappa]$ is $\kappa$-presentable). Now, a simple way to get accessibility of all fibers is to appeal the results of \cite[Ch. 5]{MP89} (in particular, all 2-limits of accessible categories are accessible categories).

	Each reindexing is accessible, it follows from the assumption that all $T_A$ are accessible functors, by checking the universal property.

	As for the last condition, we have to prove that the canonical comparison functor
	\[
		\vxy{
			\Alg_\clX(\colim\, T_i) \ar[r] & \lim_i \Alg_\clX(T_i)
		}
	\]
	obtained from the cone $\alpha_i^* : T_i\To \colim\, T_i$ is in fact an equivalence. The proof is a matter of unwinding the definition and checking its universal property.

	This ensures that $\var[p]{\algTotal\params\carriers}\params$ is accessible (which means its total category is accessible, and its projection is an accessible functor).
\end{proof}
Note that the hypotheses are not as restrictive as they seem, as they allow us to cover in one swoop:
\begin{itemize}
	\item all cases in which reindexings are covariant: co\textEM opfibrations, Kle\-i\-sli opfibrations, endofunctor coalgebras\dots; this can also be appreciated directly, relying on the completeness theorem for the 2-category of accessible categories, and presenting the the relevant opfibrations as pullbacks of accessible functors over $\en\clX[<\kappa]$;
	\item the fibrations of endofunctor algebras over accessible categories, cf.\  \autoref{swindle_theorem};
	\item \textEM fibrations: notably, the proof of \autoref{swindle_theorem} can be carried over unchanged, and $s_\infty$ will be an \textEM algebra assuming $S,T$ are monads. But there is a slicker argument in that case: from \cite[4.3.2]{Bor2} we know that a category $\clC^T$ of \textEM algebras for a monad $T : \clC\too\clC$ has all colimits that $T$ preserves. Then, it will immediately follow from the monadicity result that if $\clA\times\clX\too \clA\times\clX : (A,X)\mapsto (A, T_AX)$ preserves colimits of shape $\clJ$, then $\emalg\clA\clX$ has colimits of shape $\clJ$.
\end{itemize}


\subsection{Actegories and the semidirect product intuition}\label{subsec:act}
It turns out that when $\params$ admits coproducts, one can consider \emph{lax} monoidal functors $(\params,+)\too\carriers$. (This could be called a \defn{lax }$(\params,+)$\defn{-actegory}.)
It was indeed pointed out in \cite{BJK:internal_object_actions} that there is an equivalence of categories between
\begin{itemize}
	\item lax monoidal functors of type $(\params,+)\too\en\carriers$;
	\item functors $\params\too\Mnd\carriers$.\footnote{If $\clX$ admits enough colimits so that $\Mnd\carriers$ has coproducts, this latter category is in turn equivalent to the category of coproduct preserving functors $\params^\coprod\too\Mnd\carriers$, where $\params^\coprod$ is the free coproduct completion of $\params$, but we will not need this further characterization. Another characterization that we will not need is that these equivalence of categories are in fact equivalences of 2-categories.}
\end{itemize}
The equivalence is easy to describe explicitly: given a functor $F  : \params \to \Mnd{\carriers}$, one defines laxators
\[
	F_A\circ F_B \xRightarrow{\iota_A \circ \iota_B}  F_{A+B}\circ F_{A+B} \xRightarrow{\mu^{A+B}}  F_{A+B}
\]
and a unitor $\eta^\varnothing : \id\carriers\To F_\varnothing$ is given by the unit of the monad $F_\varnothing$. Vice versa, any lax monoidal functor $F  : (\params,+)\to (\en\carriers ,\circ)$ lets us consider each $F_A$ as monad with multiplication
\[
	\vxy{F_A\circ F_A \ar@{=>}[r] & F_{A+A} \ar@{=>}[r] & F_A.}
\]
Now, each monoidal category $(\params,\otimes)$ equips the endo-2-functor $\params \times \firstblank$ of $\Cat$ with the structure of a $2$-monad, the (lax, pseudo, strict) algebras of which are precisely the (lax, pseudo, strict) $(\params,\otimes)$-actegories. This is a banality: monoidal categories are precisely pseudomonoids in $\Cat$; also, this is just the 2-dimensional, lax analogue of Example~\ref{example_2}.

Restricting our attention to coCartesian monoidal categories, this point of view allows us to see the category of parametrized monads as the 2-category $\coCartCat \ltimes^\ell \Cat$ of lax actegories over coCartesian monoidal categories, corresponding to the parametrized $2$-monad
\[
	\coCartCat \to \text{2-}\Mnd{\Cat} \,, \quad \clA \mapsto \clA \times \firstblank
\]
that the cocartesian monoidal structure on the categories induces.
\color{red}
\color{black}
\begin{remark} \label{remark:_comonad_algebras}
	One could get around the annoyance of being restricted to coCartesian categories of parameters $\params$ by considering the following variation of the construction.
	The coCocartesian monoidal structure $+:\params \times \params \to \params$ is left adjoint to the (essentially unique) pseudocomonoid structure given by the diagonal $\Delta : \params \to \params \times \params$, which will induce the parametrized $2$-comonad analogue of Example~\ref{fib_reg_rep} on $\params \times \firstblank$.

	Due to $+$ and $\Delta$ being adjoint, the lax algebras of the parametrized $2$-monad $\params \times \firstblank$ are in bijection with the lax \textEM coalgebras of the parametrized $2$-comonad $\params \times \firstblank$. While the use of lax algebras instead of lax coalgebras for a $2$-comonad is a non-standard notion, in this example these lax algebras correspond precisely to parametrized monads, with the additional benefit that the $2$-comonad structure on $\params \times \firstblank$ doesn't require $\params$ to be cocartesian.
\end{remark}

Taking \autoref{remark:_comonad_algebras}, or by direct construction, we can consider the total category $\Cat \ltimes^\ell \Cat$ of all parametrized monads, which allows us to consider the 2-functor
\[
	\Cat \ltimes^\ell \Cat \xrightarrow{\ltimes} \Cat
\]
that maps a parametrized monad to the total category of the fibration of \textEM algebras. At an informal level, we can consider this as an instance of the `micro-macrocosm principle': a construction of a certain type (the semidirect product of monoids) arises as a functor defined from a domain of a similar `semidirect product' form. 
% \begin{remark} \label{remark:copower_action_of_monoids}
 % The semidirect product of monoids described in \autoref{ltimes_from_ltimes_mon} as a functor
	% \[
	% 	\vxy{
	% 		\emalg\firstblank\firstblank :\algTotal\Mon\Mon \ar[r] & \Mon \,,
	% 	}
	% \]
	% has domain the total category of the \textEM fibration of the parametrized monad $T  : \Mon \to \Mnd{\Mon}$, where
	% \[
	% 	T_A X  \coloneqq A \cdot X = \sum_{a \in A} X
	% \]
	% acts by copowering a monoid $X$ with the set $A$, and $T_A$ gains its monad structure from the monoid structure on $A$.
% \end{remark}
\begin{remark}[On the relation with graded monads]\label{rel_grad_mona}
	Lax monoidal functors from a one-object bicategory are sometimes also called \emph{graded monads}; they have their own notion of algebra, different from ours (cf. \cite[Definition 5.1]{Dorsch2018GradedMA}). The category of algebras of a lax monoidal functor $(\params,+) \to \en\carriers$, considered as a graded monad, is calculated as the \emph{lax limit} of the lax functor $(\params,+) \to \Cat$, which has no evident associated fibration over $\params$.

	A comparison between graded monads and parametrized monads (and thus, implicitly, with our framework) can be found in \cite{fujii20192categorical}. In a few words, our theory of fibrations of \textEM algebras relates with the fairly well-developed theory of graded monads as follows:
	\begin{itemize}
		\item we do not require the representation $T : \params \too \Mnd\carriers$ to be monoidal, \ie we do not require that $T$ lifts to a lax functor from a bicategory --a mere category suffices;
		\item we do not consider algebras for all parameters at once, as in \cite{milius_et_al:LIPIcs:2015:5538,Dorsch2018GradedMA}, but instead for each object separately.
	\end{itemize}
	The second point deserves more explanation and sheds light on the precise comparison between the two concepts: recycling a technique from \cite[Definition 1.2]{Ozornova2021} it is possible to define a certain bicategory $\Sigma\params$ (circumventing the absence of a monoidal product in $\params$) called the \emph{suspension} of $\clA$, such that parametrized monads $T : \params\times\carriers\too\carriers$ are classified by lax functors $\bar T$ out of $\Sigma\clA$:
	\[\Cat(\params,\Mnd\carriers)\cong \textbf{Lax}(\Sigma\params,\Cat)\]
	given a diagram $\params^\op\to \Cat : A\mapsto \EM(T_A)$, the lax limit of $\bar T : \Sigma\params\to\Cat$ is precisely $\algTotal[\EM]{\clA}{\clX}$. 
 
 This note does not further analyze the consequences of this remark, as no example or application gets easier when $T$ is replaced by $\bar T$; but in a forthcoming, more comprehensive work, we plan to delve deeply into the two-dimensional aspects of this topic.
	% \greta{By this we mean that we are better because here there is? Even if that's not the case, we need a bottom line here.}
	% \fosco{Heh, I am not convinced either: in my view, graded monads and diparametrized ones go together as `comparison with what other people have interpreted as parametric stuff'}
	% \greta{Fair enough, then I think we should consider moving this somewhere else (even if it's in the introduction, and we say `this is different from...'). We should do it when the overall structure is definitive, though.}
\end{remark}
%\ulo{In the above, perhaps make things more clear (the total category of the fibration of algebras is the lax limit, not the pseudofunctor $\clA^\op \too \Cat$.)}
We end the section pointing out an example that substantiates our intuition of $\emalg\Grp\Grp$ as a higher-dimensional version of a semidirect product: the semidirect product operation happens to be a functor with domain $\emalg\Grp\Grp$, and furthermore a left adjoint. Here we construct $\emalg\Grp\Grp$ as in \autoref{remark:copower_action_of_monoids}, starting from parametrized monad that acts via copowering.


\begin{proposition}\label{ltimes_from_ltimes_grp}
	Let $G$ be a group, and $\alpha : G\times G\to G$ be the conjugation action $(g,h)\mapsto g^{-1}hg$ of $G$ on itself.
	Then, there is a functor
	\[
		\vxy{
			r_\alpha : \Grp \ar[r] & \emalg\Grp\Grp
		}
	\]
	sending $G$ to the object $(G,\alpha)^G\in\emalg\Grp\Grp$. The functor $r_\alpha$ has a left adjoint, sending a $G$-group $(H,\psi)^G$ to the \emph{semidirect product} $G\ltimes_\psi H$.
\end{proposition}
\begin{proof}
	A group homomorphism $\varphi : G\to H$ defines a morphism $(\varphi,\varphi) : (G,\alpha_G)^G\to (H,\alpha_H)^H$ of algebras, because the diagram
	\[\vxy{
		G\cdot G \ar[d]_{\alpha_H} \ar[r]^-{\varphi\cdot\varphi}& H\cdot H\ar[d]^{\alpha_H} \\
		G \ar[r]_\varphi & H
		}\]
	commutes, if $\varphi\cdot\varphi$ is defined as $G\cdot G \xto{G\cdot\varphi} G\cdot H \xto{\varphi\cdot H} H\cdot H$. This defines $r_\alpha$ on morphisms, and clearly composition and identities are preserved.

	The left adjoint to $r_\alpha$ is now defined in terms of the semidirect product operation of groups; let's show that $(H,\psi)^G\mapsto G\ltimes_\psi H$ is indeed a functor $\emalg\Grp\Grp\too\Grp$:
	\begin{itemize}
		\item morphisms in $\emalg\Grp\Grp$ are pairs of maps $(u,f) : (H,\psi)^G\to (K,\theta)^{G'}$ such that
		      \[\label{mor_in_emalg_Grp}\vxy{
				      G\times H\ar[d]_\psi\ar[r]^{u\times f} & G'\times K \ar[d]^\theta\\
				      H \ar[r]_{f} & K
			      }\]
		      Every such morphism induces a function $u\ltimes f : G\ltimes_\psi H\to G'\ltimes_\theta K$ between the semidirect products, defined sending $(g,h)\in G\ltimes_\psi H$ to $(ug,fh)$; evidently the identity of $G\ltimes_\psi H$ is preserved, and given how the composition operation is defined this is a group homomorphism:
		      \begin{align*}
			      (u\ltimes f)((g_1,x)\cdot(g_2,y)) & = (u\ltimes f)(g_1.g_2,\psi(g_2,x).y) \\
			                                        & =(u(g_1.g_2),f(\psi(g_2,x).y))        \\
			                                        & =(u(g_1).u(g_2),f(\psi(g_2,x)).fy)    \\
			                                        & =(u(g_1).u(g_2),\theta(ug_2,fx).fy)   \\
			                                        & =(ug_1,fx)\cdot(ug_2,fy)
		      \end{align*}
		\item composition and identities in $\emalg\Grp\Grp$ are preserved by this definition.
	\end{itemize}
	Now, to prove that there is an adjunction $\_\ltimes\_ \dashv r_\alpha$, one can establish the bijection
	\[\emalg\Grp\Grp\big((H,\psi)^G,(G',\alpha)^{G'}\big)\cong
		\Grp(G\ltimes_\psi H, G')\]
	natural in all its arguments. This essentially follows from how a morphism $(u,f) : (H,\psi)^G\to (K,\theta)^{G'}$ is defined in \eqref{mor_in_emalg_Grp}.
\end{proof}
\begin{remark}\label{ltimes_from_ltimes_mon}
	In a similar vein, the semidirect product \emph{of monoids} \cite[3.9]{Janelidze+2003+99+114}, \cite[3.2]{Bourn1998} can be characterised as a functor
	\[
		\vxy{
			\emalg\firstblank\firstblank :\algTotal\Mon\Mon \ar[r] & \Mon \,,
		}
	\]
	having domain the total category of the \textEM fibration of the parametrized monad $T  : \Mon \to \Mnd{\Mon}$, where
	\[
		T_A X  \coloneqq A \cdot X = \sum_{a \in A} X
	\]
	acts by copowering a monoid $X$ with the set $A$, and $T_A$ gains its monad structure from the monoid structure on $A$.
 
	This functor preserves all colimits, as the semidirect product $M\ltimes_\phi N$ obtained from a representation $\phi : M\times N \to N$ via monoid homomorphisms is the coequalizer of the diagram
	\[
		\vxy{
			M\times N \ar@<.4em>[r]\ar@<-.4em>[r]& M*N \ar[r] & M\ltimes N
		}
	\]
	where the upper map is defined as $(m,n)\mapsto [m,a(m,n)]$ (seen as equivalence class of a word in $M*N$) and the lower map as $(m,n)\mapsto [n,m]$.

	It can be shown that $\emalg\Mon\Mon$ is locally presentable (using techniques from \cite{MP89}), and thus $\barealg\firstblank\firstblank$ is a left adjoint. Note how it might be difficult to establish its right adjoint explicitly, as the conjugation representation of \autoref{ltimes_from_ltimes_grp} doesn't exist for monoids.
\end{remark}

